OpenTag: Open Attribute Value Extraction from Product Profiles [Deep Learning, Active Learning, Named Entity Recognition]

Extraction of missing attribute values is to find values describing an attribute of interest from a free text input. Most past related work on extraction of missing attribute values work with a closed world assumption with the possible set of values known beforehand, or use dictionaries of values and hand-crafted features. How can we discover new attribute values that we have never seen before? Can we do this with limited human annotation or supervision? We study this problem in the context of product catalogs that often have missing values for many attributes of interest. In this work, we leverage product profile information such as titles and descriptions to discover missing values of product attributes. We develop a novel deep tagging model OpenTag for this extraction problem with the following contributions: (1) we formalize the problem as a sequence tagging task, and propose a joint model exploiting recurrent neural networks (specifically, bidirectional LSTM) to capture context and semantics, and Conditional Random Fields (CRF) to enforce tagging consistency, (2) we develop a novel attention mechanism to provide interpretable explanation for our model's decisions, (3) we propose a novel sampling strategy exploring active learning to reduce the burden of human annotation. OpenTag does not use any dictionary or hand-crafted features as in prior works. Extensive experiments in real-life datasets in different domains show that OpenTag with our active learning strategy discovers new attribute values from as few as 150 annotated samples (reduction in 3.3x amount of annotation effort) with a high F-score of 83%, outperforming state-of-the-art models.

==> attention.tex <==
\section{Self Attention Mechanism}\label{sec:attention}
\subsection{Overall Architecture}


A recent trend in deep learning is attention mechanism.
It is loosely based on the visual attention mechanism found in humans.
Although there exist different models for attention mechanism, all of them essentially come down to being able to focus on a certain region of an image with ?high resolution? while perceiving the surrounding image in ?low resolution?, and then adjusting the focal point over time.

The recent biggest success of attention mechanism is its use in Neural Machine Translation (NMT).
Currently, most NMT systems have the structure of sequence to sequence which is comprised of encoder and decoder.
The meaning of a sentence is mapped into a fixed-length vector representation by an encoder and then the translation is generated based on that vector by a decoder.
In the very original version of NMT model the decoder is supposed to generate a translation solely based on the last hidden state.
But it seems somewhat unreasonable to assume that we can encode all information about a potentially very long sentence into a single vector and then have the decoder produce a good translation based on only that. 
With an attention mechanism we no longer try encode the full source sentence into a fixed-length vector.
Rather, we allow the decoder to ?attend? to different parts of the source sentence at each step of the output generation.
Importantly, we let the model learn what to attend to based on the input sentence and what it has produced so far.

The intuition behind the attention mechanism is that for each step, we will replace the current hidden state with a weighted summation of all the input tokens.
The weight will be calculate by align the current hidden state which represent the semantic it has produced so far and each word token of input sequence.
As a result, attention mechanism is essentially an align model which requires two objects to align with each other.
However, there is not current hidden state in our case, which can be used to align with the input tokens due to the lack of decoder.
We have to make a little modification to the existing align model.
We apply a non-linear transformation to the hidden vectors of each token and use them to align with all the tokens include itself, thus deriving a self-attention mechanism.
Similar ideas have been proposed in 

\subsection{Self Attention Module}
\subsection{Formal Definition}
\subsection{Derive Explanations}
